Polybot: Training One Policy Across Robots While Embracing Variability

Reusing large datasets is crucial to scale vision-based robotic manipulators to everyday scenarios due to the high cost of collecting robotic datasets. However, robotic platforms possess varying control schemes, camera viewpoints, kinematic configurations, and end-effector morphologies, posing significant challenges when transferring manipulation skills from one platform to another. To tackle this problem, we propose a set of key design decisions to train a single policy for deployment on multiple robotic platforms. Our framework first aligns the observation and action spaces of our policy across embodiments via utilizing wrist cameras and a unified, but modular codebase. To bridge the remaining domain shift, we align our policy's internal representations across embodiments through contrastive learning. We evaluate our method on a dataset collected over 60 hours spanning 6 tasks and 3 robots with varying joint configurations and sizes: the WidowX 250S, the Franka Emika Panda, and the Sawyer. Our results demonstrate significant improvements in success rate and sample efficiency for our policy when using new task data collected on a different robot, validating our proposed design decisions. More details and videos can be found on our anonymized project website: https://sites.google.com/view/polybot-multirobot

==> rss/defs.tex <==
\newcommand{\x}{\mathbf{x}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\data}{\mathcal{D}}

\newcommand{\etal}{{et~al.}\ }
\newcommand{\eg}{\emph{e.g.},\ }
\newcommand{\ie}{\emph{i.e.},\ }
\newcommand{\nth}{\text{th}}
\newcommand{\pr}{^\prime}
\newcommand{\tr}{^\mathrm{T}}
\newcommand{\inv}{^{-1}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\gauss}{\mathcal{N}}
\newcommand{\norm}[1]{\left|#1\right|}
\newcommand{\trace}{\text{tr}}

%% specifics for the paper
\newcommand{\reward}{r}
\newcommand{\policy}{\pi}
\newcommand{\mdp}{\mathcal{M}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\actions}{\mathcal{A}}
\newcommand{\observations}{\mathcal{O}}
\newcommand{\transitions}{P}
\newcommand{\initstate}{d_0}
\newcommand{\freq}{d}
\newcommand{\obsfunc}{E}
\newcommand{\initial}{\mathcal{I}}
\newcommand{\horizon}{H}
\newcommand{\rewardevent}{R}
\newcommand{\probr}{p_\rewardevent}
\newcommand{\metareward}{\bar{\reward}}
\newcommand{\discount}{\gamma}
\newcommand{\behavior}{{\pi_\beta}}
\newcommand{\bellman}{\mathcal{T}}
\newcommand{\qparams}{\phi}
\newcommand{\qparamset}{\Phi}
\newcommand{\qset}{\mathcal{Q}}
\newcommand{\batch}{B}
\newcommand{\qfeat}{\mathbf{f}}
\newcommand{\Qfeat}{\mathbf{F}}
\newcommand{\hatbehavior}{\hat{\pi}_\beta}

\newcommand{\traj}{\tau}

\newcommand{\pihi}{\pi^{\text{hi}}}
\newcommand{\pilo}{\pi^{\text{lo}}}
\newcommand{\ah}{\mathbf{w}}

\newcommand{\proj}{\Pi}

\newcommand{\loss}{\mathcal{L}}
\newcommand{\eye}{\mathbf{I}}

\newcommand{\model}{\hat{p}}

\newcommand{\pimix}{\pi_{\text{mix}}}

\newcommand{\pib}{\bar{\pi}}
\newcommand{\epspi}{\epsilon_{\pi}}
\newcommand{\epsmodel}{\epsilon_{m}}

\newcommand{\return}{\mathcal{R}}

%% math
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\en}{\mathcal{E}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\boldm}{\mathbf{m}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\ot}{\bo_t}
\newcommand{\st}{\bs_t}
\newcommand{\at}{\ba_t}
\newcommand{\op}{\mathcal{O}}
\newcommand{\opt}{\op_t}
\newcommand{\kl}{D_\text{KL}}
\newcommand{\tv}{D_\text{TV}}
\newcommand{\ent}{\mathcal{H}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\byk}{\mathbf{y_k}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bO}{\mathbf{O}}

\newcommand{\bzhi}{\bz^\text{hi}}
\newcommand{\expected}{\mathbb{E}}
\newcommand{\srank}{\text{srank}}
\newcommand{\rank}{\text{rank}}
\newcommand{\deepnet}{\bW_N(k, t) \bW_\phi(k, t)}
\newcommand{\features}{\bW_\phi(k, t)}
\newcommand{\stateactioni}{[\bs_i; \ba_i]}
\newcommand{\diag}{\text{\textbf{diag}}}
\newcommand{\cosine}{\text{cos}}
\newcommand{\subopt}{\mathsf{SubOpt}}
\newcommand{\hatpi}{\hat{\pi}}
\newcommand{\variance}{\mathbb{V}}
\newcommand{\indicator}{\mathbb{I}}
\newcommand{\sign}{\mathsf{sign}}

\def\thetaP{\theta^{\prime}}
\def\cf{\emph{c.f.}\ }
\def\vs{\emph{vs}.\ }
\def\etc{\emph{etc.}\ }
\def\Eqref#1{Equation~\ref{#1}}

\newcommand{\E}[2]{\mathbb{E}_{#1} \left[#2\right]}
\newcommand{\condE}[2]{\mathbb{E} \left[#1 \,\middle|\, #2\right]}
\newcommand{\Et}[1]{\mathbb{E}_t \left[#1\right]}
\newcommand{\prob}[1]{\mathbb{P} \left(#1\right)}
\newcommand{\condprob}[2]{\mathbb{P} \left(#1 \,\middle|\, #2\right)}
\newcommand{\probt}[1]{\mathbb{P}_t \left(#1\right)}
\newcommand{\var}[1]{\mathrm{Var} \left[#1\right]}
\newcommand{\condvar}[2]{\mathrm{Var} \left[#1 \,\middle|\, #2\right]}
\newcommand{\std}[1]{\mathrm{Std} \left[#1\right]}
\newcommand{\condstd}[2]{\mathrm{Std} \left[#1 \,\middle|\, #2\right]}

\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\ceils}[1]{\left\lceil#1\right\rceil}
\newcommand{\floors}[1]{\left\lfloor#1\right\rfloor}
\newcommand{\I}[1]{\mathds{1} \! \left\{#1\right\}}

\def\polylog{\operatorname{polylog}}

\newenvironment{repeatedthm}[1]{\@begintheorem{#1}{\unskip}}{\@endtheorem}

% \DeclareMathOperator\supp{supp}
\newcommand{\methodname}{CDS}
\newcommand{\aliasingproblemname}{bootstrapping aliasing}
\newcommand{\Aliasingproblemname}{Bootstrapping aliasing}
\newcommand{\AliasingProblemName}{Bootstrapping Aliasing}
\newcommand{\simnorm}{\mathrm{sim}_{\mathrm{n}}^\pi}
\newcommand{\simunnorm}{\mathrm{sim}_{\mathrm{u}}^\pi}
\newcommand{\taustar}{\tau^*}

\newcommand\disteq{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny D}}}{=}}}

\newcommand{\doubt}[1]{\textcolor{magenta}{#1}}

==> rss/text/0-abstract.tex <==
\begin{abstract}
% final cutting version 

% While reinforcement learning (RL) has shown remarkable success in solving simulated sequential decision-making problems, applying RL to embodied robotic agents is far more challenging. 
Reinforcement learning (RL) algorithms typically require a substantial amount of data, which may be time-consuming to collect with a robot, as well as the ability to freely return to an initial state to continue practicing a task, which requires laborious human intervention in the real world. Moreover, robotic policies learned with RL often fail when deployed beyond the carefully controlled setting in which they were learned. 
In this work, we demonstrate that these varied challenges of real-world robotic learning can all be tackled by effective utilization of diverse offline interaction datasets collected from previously seen tasks. 
While much prior work on robotic RL has focused on learning from scratch, and has attempted to solve each of the above problems in isolation, 
we devise a system that uses prior offline datasets to tackle all of these challenges together. 
Our system first uses techniques from offline reinforcement learning to extract useful skills and representations from prior offline data, which gives the agent a baseline ability to perceive and manipulate the world around it. 
Then, when faced with a new task, our system adapts these skills to quickly learn to both perform the new task \emph{and} return the environment to an initial state, effectively learning to perform its own environment reset. We show that training on prior data gives rise to behaviors that generalize to far more varied conditions, than simply not using this data. 
We evaluate our method on a suite of challenging robotic manipulation tasks, involving high-dimensional visual observations and sparse binary reward functions, both in the real world and in simulation. 
Our empirical results demonstrate that incorporating prior data into robotic reinforcement learning enables autonomous learning, substantially improves sample-efficiency of learning, and results in policies that generalize better. 

% While reinforcement learning (RL) has shown remarkable success in solving simulated sequential decision-making problems, applying RL to embodied robotic agents is far more challenging. 
% RL algorithms typically require a substantial amount of data, which may be time-consuming to collect with a robot, as well as the ability to freely return to an initial state to continue practicing the task, which requires laborious human intervention in the real world. Moreover, robotic policies learned with RL often fail when deployed beyond the carefully controlled setting in which they were learned. 
% In this work, we demonstrate that these varied challenges of real-world robotic learning can all be tackled by effective utilization of diverse offline interaction datasets collected from previously seen tasks, under different physical conditions, and even on different robotic systems. 
% While much prior work on robotic RL has focused on learning from scratch, and has attempted to solve each of the above problems in isolation, 
% we devise a system that uses prior offline datasets to tackle all of these challenges together. 
% Our system first uses techniques from offline reinforcement learning to extract useful skills and representations from prior offline data, which gives the agent a baseline ability to perceive and manipulate the world around it. 
% Then, when faced with a new task or test condition, our system adapts these skills to quickly learn to both perform the new task \textit{and} return the environment to an initial state, effectively learning to perform its own environment reset. We show that training on prior data gives rise to behaviors that that generalize to far more varied conditions, than simply not using this data. 
% We evaluate our method on a suite of challenging robotic manipulation tasks, involving high-dimensional visual observations and sparse binary reward functions, both in the real world and in simulation. 
% Our empirical results demonstrate that incorporating prior data into robotic reinforcement learning enables autonomous learning, substantially improves sample-efficiency of learning, and results in policies that generalize better. 


%%AK: Avi's draft version
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In this work, our key insight is the following: the varied challenges of real world robotic learning can be tackled through more effective utilization of interaction datasets from previously seen tasks. 
% While much prior work on robotic RL has focused on learning from scratch, this does not match how humans learn. When confronted with a new task, we exploit our prior knowledge of similar tasks to quickly identify optimal behaviors, scaffold learning, and generalize to different variations of the problem. 
% We devise a robotic system that similarly leverages experience gained from solving previous tasks to learn new tasks more efficiently and autonomously. 
% Our system uses offline RL to extract useful skills and representations from a dataset of prior experience. 
% Then, when faced with a new task, our system adapts these skills to quickly learn to both perform the new task \textit{and} return the environment to an initial state distribution, effectively learning to perform its own environment reset. 
% We also find that by initializing with prior data, our system learns behaviors that generalize to far more varied conditions. 
% % In summary, we demonstrate that incorporating prior data into robotic reinforcement learning enables autonomous learning, and improves sample-efficiency and generalization.
% We evaluate our method on a suite of challenging robotic manipulation tasks, involving high-dimensional visual observations and sparse reward functions, both in the real world and in simulation. 
% Our results demonstrate that incorporating prior data into robotic reinforcement learning enables autonomous learning, substantially improves sample-efficiency of the learning, and results in policies that generalize better. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%









% Applying rl to robots is hard because requires lots of data, manual resets, and careful instrumentation of the environment because policies don't generalize

% However, while typically learning is applied to robots from scratch this doesn't match how humans and animals learn

% We bring our prior knowledge to bear on new problems which allows us to solve them efficiently, generalize to different variations of the problem, and use prior skills to return the environment to an initial state

% We devise a robotic learning system that similarly leverage prior experience solving to learn a new problem more effectively.

% We use offline data from strutrually similar prior tasks to initialize the learning on a new task, giving sample efficiency

% We use the prior data to intialize both a forward and backward controller, enabling autonomous learning

% We show that leveraging prior data in this way additionally results in learning robust behaviors that generalize to different conditions better than policies learned without access to prior data. 
\end{abstract}

==> rss/text/1-introduction.tex <==
\section{Introduction}
Reinforcement learning (RL) provides a concise and appealing abstraction that captures the problem of learning behavioral skills for embodied systems such as robots: by framing the problem as experiential utility maximization, RL provides a general learning-based framework that, in principle, could be utilized to acquire any goal-directed behavior. However, in practice, the standard RL problem formulation overlooks many of the challenges that arise in real-world robotic learning. RL problems are classically (though not exclusively) situated in settings where ample exploration can be performed from scratch, the environment can be reset episodically, and the focus is more on attaining the highest possible performance rather than good generalization, as for example in the case of playing a board game or video game. However, real-world robotic learning problems have very different constraints. With real-world robots, online interaction and exploration is often at a premium, the robot must figure out how to reset the environment itself between attempts, and the natural variability and uncertainty of the real world makes generalization far more essential than squeezing out every bit of final performance. 

Of course, humans and animals that must also deal with the real world also need to handle each of these challenges. However, in contrast to standard robotic RL settings, humans do not approach each new problem with a blank slate: we leverage prior experience to help us acquire new skills quickly, scaffold the process of learning that skill (e.g., by using skills we already have to practice and try again), and utilize representations learned from prior experience to ensure that the new skill is represented in a robust and generalizable way. We study an analogous approach in this work: while prior work has discussed many of the challenges associated with real world robotic learning in isolation, and proposed individual technical solutions \cite{eysenbach2017leave, han2015learning, ha2020learning, zhu2020ingredients, xu2020continual, gupta2021reset, sharma2021autonomoussubgoal, lu2020reset, kalashnikov2018qt, kalashnikov2021mt, cabi2019scaling, nair2020accelerating}, we instead ask whether all of these issues can be alleviated by appropriately incorporating prior data. Our central thesis is that prior experience that the robot collected for performing a variety of other related tasks can facilitate many seemingly distinct aspects of autonomous robotic learning, including better sample-efficiency, better generalization of skills learned in a narrow setting, and learning with infrequent resets.

\begin{figure}[!t]
    \label{fig:overview}
    \centering
    \includegraphics[width=\linewidth]{figures/fig1_v5.pdf}
    \caption{\textbf{Overview of our system.} In the offline stage (left), we train a multi-task policy that captures prior knowledge from an offline dataset of previously experienced tasks. Then, in the online stage (right), this multi-task policy is used to initialize learning for a new task, providing both a forward policy and a backward (reset) skill, and improving learning speed and generalization. We demonstrate that this approach leads to sample-efficient learning of generalizable policies with a significant reduction in the need for manual interventions (i.e., resets).}
    %%SL.1.17: Generally this sketch is a good starting point for the figure, but I suggest a few improvements: (i) somehow make it clearer how the left side connects to the right side -- right now they seem completely disconnected from one another; (ii) it would be good if this figure had some pictures of robots in it, so that it serves the dual role both of providing a diagram of the approach and showing some pictures of what's going on, then we can put this on page 1 and it would also serve as a teaser and get across the point that the paper is about real robots
    %%SL.1.26: We really should try to make some forward progress toward finalizing this figure. Ideally also get it on page 1. A great opening figure is important for making a good first impression.
    %%AY.1.27: Inserted draft. Not great yet but attempts to address (i) and (ii).
    %%HW.1.28 Could we get something in this figure to represent that finetuning occurs with minimal resets? Also do we need to show the value function here? We can maybe fix the sizing by making all text, images, and icons bigger and lines thicker.
    \label{fig:my_label}
\end{figure}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/teaser_v0.pdf}
%     \caption{TODO}
%     \label{fig:teaser}
% \end{figure}

The strategy of accelerating learning by initially pretraining on a broad prior dataset is supported by the widespread success of pretraining and finetuning in supervised learning. Prior work in computer vision and natural language processing has demonstrated that pretraining on large and diverse datasets enables both data efficiency and broad generalization \cite{brown2020language, huh2016makes, radford2021learning, bommasani2021opportunities}. Thus, extending the idea of pretraining on diverse data to robotics is a natural step towards more effective real-world learning. With the goal of taking a data-driven approach to robotics, prior work has explored offline RL to leverage static datasets~\cite{peters2007reinforcement, kalashnikov2018qt, wu2019behavior, fujimoto2019off, kumar2019stabilizing, peng2019advantage, wang2020critic, kumar2020conservative, nair2020accelerating, fujimoto2021minimalist, kostrikov2021offline, kostrikov2021iql}, multi-task and meta RL to handle diverse multi-task data~\cite{wilson2007multi, parisotto2015actor, teh2017distral, espeholt2018impala, hessel2019multi, yu2020gradient, xu2020knowledge, yang2020multi, sodhani2021multi, kalashnikov2021mt, yu2021conservative}, and reset-free learning to collect data autonomously~\cite{eysenbach2017leave, han2015learning, ha2020learning, zhu2020ingredients, xu2020continual, gupta2021reset, sharma2021autonomoussubgoal, lu2020reset}.
%%SL.1.10: Some of this will be pretty redundant with the related work section. That's maybe OK, but if we end up short on space, consider shortening some of the above prior work discussion.
However, addressing the full real-world learning problem, as we discussed before, requires not only algorithms for learning from prior data, but the right system that combines these algorithms into a multi-task, reset-free framework. To this end, we propose a complete system for extracting useful skills from prior data and applying them to learn new tasks autonomously. Although the individual components of our system are based on previously proposed principles and methods for offline RL~\cite{nair2020accelerating}, multi-task learning with task embeddings~\cite{kalashnikov2021mt, hausman2018learning}, and reset-free learning with forward-backward controllers~\cite{han2015learning, eysenbach2017leave, zhu2020ingredients, xu2020continual, sharma2021autonomoussubgoal}, our system combines these components into a novel framework that effectively enables real-world robotic learning and leverages prior data for all of these parts.

Our system consists of two phases: offline learning using the prior data, and mostly autonomous online finetuning on a new task (see Figure \ref{fig:overview}), where only occasional resets are provided. In the offline phase, our goal is to extract skills and representations from the prior data that may be useful on the new task. Accordingly, we use an offline RL algorithm to obtain a multi-task policy capable of performing the different behaviors in the offline data. Then, in the online phase, we adapt the learned skills to the new task. To enable autonomous learning, we finetune two distinct skills for each new task, alternating between attempting the task and resetting the environment. If the behaviors required to perform the target task and reset the environment are structurally similar to those in the prior data, the skills learned offline will succeed at performing and resetting the task with non-negligible probability, providing a learning signal that allows the agent to adapt its behavior with only a small amount of online data. Moreover, initially training on a broad dataset of experience encourages learning representations that are robust to axes of variation that are irrelevant to performing the task. Where polices learned from narrow data may overfit to unimportant details of the environment and fail when those details change, polices learned from diverse multi-task data can generalize to new conditions with little to no adaptation.



%%SL.1.3: This paragraph should explicitly state what the contribution is. Generally, I would recommend spending more time to refine this paragraph to make it crisp and also more compelling. It needs to very clearly tell the reader what the new thing is that this paper does that prior papers don't do.
Our main contribution is demonstrating that incorporating prior data into a reinforcement learning setup simultaneously addresses several key challenges in real-world robotic RL: sample-efficiency, zero-shot generalization, and autonomous non-episodic learning. Prior work has addressed parts of the real-world learning problem with specific technical solutions, but we build a complete system for robotic reinforcement learning that leverages prior data.
The individual components of our system, such as the choice of RL algorithm, are not novel, but the combination of these parts is a system with novel capabilities to bootstrap effective real-world online RL with multi-task prior data.
We validate our approach on real-world robotic manipulation, where we show that our method makes it possible to learn to manipulate new objects via RL in settings where prior approaches struggle to make progress, reach final performance that is comparable to what the algorithm can attain when provided with ``oracle'' demonstration data for the new task, and acquire policies that generalize more broadly than those trained only on single-task data.
%%SL.1.28: I somewhat rewrote the experimental claims, double-check please that the above stuff is still correct
%We validate our approach on robotic manipulation tasks and demonstrate that our system achieves comparable or superior performance to prior work that addresses sample-efficiency, generalization, and reset-free learning separately. Our system solves the manipulation tasks in our evaluation with Ax fewer environment resets, Bx fewer samples, and generalizes to a broader range of tasks than approaches that do not use prior data. [insert more concrete details about what we end up achieving here]

%%SL.1.26: Something that we need to make sure not to forget: if the final method is not fully autonomous, let's carefully go over the intro and make sure that we are not claiming the method is fully autonomous. We may need to somewhat temper our claims and use more careful language like "only occasional resets" or something. It's very bad if we end up with claims of being "fully autonomous" or "reset-free" when in fact the method isn't.


==> rss/text/2-related-work.tex <==
\section{Related Work}
In this section we review prior work that has explored learning behaviors from offline datasets, leveraging multi-task data, and reinforcement learning with minimal resets. We build on techniques from each area to devise a complete system for automated robot learning.

\textbf{Accelerating online RL with offline data.} 
Our method is not the first to propose learning behaviors from offline data to improve the efficiency of RL. Methods for imitation learning use offline data in the form of demonstrations to learn behavior, and imitation learning can be used to accelerate reinforcement learning \cite{schaal1997learning, hester2017learning, rajeswaran2017learning, peng2018deepmimic, vecerik2017leveraging, kormushev2010robot, gupta2019relay, nair2017overcoming}. However, when the offline data is sub-optimal, offline reinforcement learning methods typically perform better \cite{peters2007reinforcement, kalashnikov2018qt, wu2019behavior, fujimoto2019off, kumar2019stabilizing, peng2019advantage, wang2020critic, kumar2020conservative, nair2020accelerating, fujimoto2021minimalist, kostrikov2021offline, kostrikov2021iql} and can also be combined with online finetuning \cite{nair2020accelerating, julian2020efficient, kalashnikov2021mt}.
We use an offline RL method to extract useful skills and representations from prior data, but our system includes additional components that allow us to use multi-task offline data and autonomously finetune the policy online by learning to both perform the task and reset. 
% However, offline RL methods typically assume the data comes from a single task. Some approaches leverage multi-task offline data to learn useful state representations \cite{yang2021representation, pinto2016supersizing}, temporally extended actions \cite{singh2020parrot, ajay2020opal}, or environment dynamics \cite{singh2020cog, ebert2018visual}, which can accelerate learning of downstream tasks.

%%SL.1.26: I feel like we need to do a better job in this paragraph of heading off the biggest criticisms about similarity to prior work. What do we think is the nearest prior method is? Perhaps it's MT-Opt, but whatever it is, I think we need to more directly address the issue. Basically, it's much better to be explicit in stating differences rather than not talk about it and have the reviewers wonder (the reviewers won't miss the similarity). If it's MT-Opt, we can say something like this: Perhaps the closest prior system to ours in this area is~\citet{}, which studies multi-task learning for a similar class of grasping-based robotic manipulation tasks. However, in contrast to this prior work, our focus is not on how to train a multi-task policy, but specifically on how prior offline data from varied tasks can be leveraged to improve the autonomy and generalization when learning a new task. While \citet{} also evaluates finetuning to new tasks, our system goes significantly further, aiming to automate resets (which the prior work does not address, instead using an instrumented bin setup), and evaluating the benefits in terms of generalization and efficiency for the new task.
\textbf{Multi-task and meta-RL.} Offline RL methods typically assume the data is labeled with rewards for a single task. Methods for multi-task RL \cite{wilson2007multi, parisotto2015actor, teh2017distral, espeholt2018impala, hessel2019multi, yu2020gradient, xu2020knowledge, yang2020multi, sodhani2021multi, kalashnikov2021mt, yu2021conservative} address the additional challenges that arise when learning from multi-task data, like sharing model parameters between tasks. Some approaches share parameters by learning a single policy conditional on a space of tasks \cite{kalashnikov2021mt, hausman2018learning}.
%or goal states in the case of goal-reaching tasks \cite{nair19ccrig, mandlekar2020iris, khazatsky2021can, chebotar2021actionable}. 
We similarly adopt the strategy of learning a task conditioned policy, however unlike multi-task RL methods our focus is adapting this multi-task policy to unseen tasks. Meta-RL methods \cite{duan2016rl, finn2017model, rakelly2019efficient, zintgraf2019varibad} share our goal of using data from prior tasks to quickly adapt to new tasks, but typically operate in the online setting. We only assume access to offline data from previous tasks. Offline meta-RL methods \cite{li2019multi, dorfman2020offline, pong2021offline, mitchell2021offline} are capable of using offline data, but do not address adaptation with minimal resets like our system.
Perhaps the closest prior system to ours in this area is~\citet{kalashnikov2021mt}, which studies multi-task learning for a similar class of grasping-based robotic manipulation tasks. However, in contrast to this prior work, our focus is not on how to train a multi-task policy, but specifically on how prior offline data from varied tasks can be leveraged to improve the autonomy and generalization when learning a new task. While \citet{kalashnikov2021mt} also evaluates finetuning to new tasks, our system goes significantly further, aiming to automate resets (which the prior work does not address, instead using an instrumented bin setup), and evaluating the benefits in terms of generalization and efficiency for the new task.





%%SL.1.10: Generally I think the above paragraph is quite good, but I'm not sure we should draw such a sharp distinction between methods that learn index-conditioned policies vs methods that learn embeddings. Perhaps we can use one term to refer to all of them (like task spaces or something?), and just say we also condition on the task (or use some other vague language like that that doesn't distinguish between indices and embeddings). The rationale for doing it this way is that our task indices thing might come off as kind of weird to some people. Once we explain it, it will be fine, but if we just say it without context, people might misunderstand and have a negative reaction. That's also why I'm not thrilled about talking about it in the intro.

% Like our method, meta reinforcement learning methods use data from prior tasks to accelerate learning on new tasks \cite{duan2016rl, finn2017model, rakelly2019efficient, zintgraf2019varibad}. Our method is most similar to context-based meta-RL methods, like PEARL \cite{rakelly2019efficient},
%%SL.1.3: It's less important to precisely describe which specific meta-learning method our approach most resembles, and more important to explain how what we're doing is different than meta-RL (or more like why meta-RL methods don't solve the problem we are solving). I think the current way of phrasing this paragraph might actually somewhat exacerbate the issue, where readers will start to wonder why our method is necessary given all the (seemingly similar) meta learning methods that are also doing a multi-task thing. But in some sense it's just a different problem.
% that learn to infer tasks from experience. On the training tasks, PEARL trains an encoder to map experience to continuous task embeddings that indicate the task to the agent, effectively learning a latent space of skills \cite{hausman2018learning}. We avoid the complexity of training a task encoder and instead use one-hot task indices to indicate the task to the agent when training on the prior data, as in multi-task RL \cite{kalashnikov2021mt}.
%%SL.1.3: This statement is risky, because it implicitly claims that it's somehow better to do this than what Hausman2018 does, but we don't really support that claim experimentally, so we shouldn't make that claim.
% When adapting to a new task, PEARL adapts the embedding via posterior sampling of the encoder, holding the sampled embedding constant throughout the episode. We similarly use a posterior sampling strategy, treating the one-hot task indices as continuous task embeddings, but we adapt the embeddings with the cross-entropy method (CEM).
%%SL.1.3: Again, this implicitly makes the claim that this is a better way to do it -- the CEM part is kind of chosen out of convenience, not because it's actually a better method, so maybe better not to draw too much attention to it at this level of abstraction.
% Meta-RL methods assume the ability to collect online data in the training environments. We only assume access to offline data from previous tasks. Offline meta-RL methods attempt to adapt online meta-RL methods to the offline setting \cite{li2019multi, dorfman2020offline, pong2021offline, mitchell2021offline}, but do not address learning without resets.
%%SL.1.3: My advice here would not to focus so much on the specific technical details about how our method is different, because then the reader will expect us to provide empirical validation that these differences are important (and helpful), but rather focus on how what we're doing is distinct from what prior multi-task and meta-RL papers solve. Be very careful here, because I think it's quite possible some reviewers will complain that we *should* have done something more like meta-RL, whereas what we did instead is somewhat simplistic (we had a good reason for doing it this way, but that's likely not apparent at this level of abstraction).

\textbf{Reset-free RL.} Our system aims to utilize prior data to autonomously learn robotic skills, leveraging prior experience to both accelerate the learning of a new behavior and the process of learning how to \emph{reset} between attempts. Prior work has tackled this ``reset-free'' learning problem \cite{sharma2021autonomous} in a number of ways. Some techniques exploit the the observation that when learning several tasks simultaneously, some tasks reset others, thus forming a curriculum \cite{gupta2021reset, lu2020reset, ha2020learning, han2015learning}. While \citet{gupta2021reset} also uses a multi-task setup to automate resets, this prior paper involves a small number of tasks that all focus on enabling reset-free learning for a particular (single) skill, whereas our focus is specifically on using prior data for \emph{other} tasks to enable a \emph{new} task to be learned as autonomously as possible.
%Our method does not assume a curriculum to scaffold learning; instead we extract useful exploratory behavior from prior data.
Other work learns separate controllers for performing the task and resetting the environment \cite{han2015learning, eysenbach2017leave, zhu2020ingredients, xu2020continual, sharma2021autonomoussubgoal}. We also learn separate controllers, but initialize them with potentially useful skills extracted from prior data. Most similar to our work, \citet{sharma2021autonomoussubgoal} use prior data in the form of demonstrations to accelerate learning forward and reset behaviors. However, our system does not rely on expert demonstrations of the target task. Instead, we use potentially sub-optimal data from other tasks.   

% Other work generates an internal curriculum by progressively expanding the region from which the agent can reset the task, choosing states to reset from based on their value under a learned value function \cite{sharma2021autonomous, eysenbach2017leave}. Our method does not assume or generate a curriculum to scaffold learning; instead we extract useful exploratory behavior from prior data. Other work avoids the difficult exploration problem of returning to a specific initial state distribution and learns to reset to a uniform state distribution, either through a novelty exploration bonus \cite{zhu2020ingredients} or an adversarial reset controller \cite{xu2020continual}. We address the more general problem of returning to a specific initial state distribution.
%%SL.1.3: My sense is that a good way to emphasize the relevant distinctions and deemphasize the less relevant distinctions is to lump zhu2020 and xu2020 in with the other general reset-free citations (since whether to use reset controller or perturbation controller is largely orthogonal to our contribution), and instead draw a distinction between forward-backward methods, methods that make a curriculum, and methods that use prior data (sharma2021, which uses demos). Remember that part of the point of this paragraph is to persuade the reader that our paper is still necessary despite all these prior papers, we should make it explicit that our central idea, in contrast to prior work, is that prior experience for *other* tasks can facilitate reset-free learning by providing a good starting point not only for a task controller but also the skills that reset it, closest is sharma2021, but it requires demos for the task being learned, whereas our method uses potentially suboptimal experience from *other* prior tasks

% \noindent \textbf{Generalization in RL.}
% Prior work on improving the zero-shot generalization capabilities of policies learned with RL has explored data augmentation, domain randomization, optimization objectives, encoding or learning invariance, regularization, and adaptation within an episode \cite{}. \citet{kirk2021survey} provides a survey. However, these methods largely apply to the online setting whereas we focus on generalization through offline datasets.
%%SL.1.3: This paragraph is quite weird. Addressing the general and extremely broad subject of generalization in RL seems kind of odd, though we could have one sentence and basically say that our method is orthogonal to these approaches and could be combined with the, but our focus is rather on how multi-task learning can facilitate better generalization and robustness for new skills (though we must empirically validate this if we're going to say that!). Overall, we should think carefully about the narrative that we want in this paragraph -- in some sense the closest prior works in this regard are going to be some of the things cited in the multi-task RL paragraph previously... it may also be that this paragraph is not necessary, or maybe this could be a place to discuss prior papers that use some representation learning from prior data or something.

%%SL.1.3: Overall, would be good to try harder to find more non-Berkeley papers in each of these sections to cite.











==> rss/text/3-preliminaries.tex <==
\section{Preliminaries}
\label{sec:prelims}
The goal in standard reinforcement learning (RL) is to learn a policy $\pi(\ba|\bs)$ that maximizes the long-term cumulative discounted reward in a Markov decision process (MDP), which is defined as a tuple $\mathcal{M} := (\mathcal{S}, \mathcal{A}, P, r, \rho, \gamma)$ where $\mathcal{S}$ is the state space, $\mathcal{A}$ is the action space, $P: \mathcal{S} \times \mathcal{A} \rightarrow \Delta(\mathcal{S})$ is the transition function, $r: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ is the reward function, $\rho \in \Delta(\mathcal{S})$ is the initial state distribution, and $\gamma \in [0, 1]$ is the discount factor. The objective in standard RL is to optimize the policy against the cumulative discounted return objective, starting from the initial state distribution $\rho$:
\begin{equation}
\label{eqn:standard_rl}
    J_\text{standard}(\pi) := \mathbb{E}_{\substack{\bs_0 \sim \rho, a_i \sim \pi, \\ \bs'_{i+1} \sim P(\cdot|\bs_i, \ba_i)}}\left[\sum_{i} \gamma^i r(\bs_i, \ba_i) \right]~~~ \text{(Standard)}.
\end{equation} 
The Q-function $Q^\pi(\bs, \ba)$ for a policy $\pi(\ba|\bs)$ is the long-term discounted reward obtained by executing action $\ba$ at state $\bs$ and following $\pi(\ba|\bs)$ thereafter. $Q^\pi(\bs, \ba)$ is the fixed point of $Q(\bs, \ba) := R(\bs, \ba) + \gamma \mathbb{E}_{\bs' \sim P(\cdot|\bs, \ba), \ba' \sim \pi(\cdot|\bs')} \left[ Q(\bs', \ba')\right]$, which is known as the Bellman equation. While the standard RL objective can be optimized in several ways,
in this work we build on the class of actor-critic methods~\citep{lillicrap2015continuous,haarnoja2018soft,kostrikov2021iql}. A typical actor-critic method alternated between two phases, policy evaluation and policy improvement. In the policy evaluation phase the current policy $\pi(\ba | \bs)$ is evaluated by fitting an action-value function ${Q}^\pi(\bs, \ba)$. In the policy improvement phase, the policy or actor $\pi(\ba | \bs)$ is updated to maximize the expected Q-value. 


% reset free RL
\textbf{Autonomous RL.} The standard RL objective is typically optimized in an ``episodic'' manner, where between each trial, the agent is reset into an initial state sampled indendently from $\rho(s)$. However, in this paper, we study the problem of {reinforcement learning with minimal external resets}, also known as autonomous reinforcement learning~\citep{sharma2021autonomous}. This requires the policy to be trained without resetting after each trial (though we do use occasional resets in our experiments). This is important in real-world settings, where it may take considerable effort to provide manual resets after every single attempt.
%The problem statement of autonomous RL requires that the policy $\pi(\ba|\bs)$ is learned in an autonomous manner, with no access to an environment-provided reset function, but is later evaluated in terms of its performance on the standard RL objective shown in Equation~\ref{eqn:standard_rl}. We will discuss the formalism of autonomous RL in the next paragraph, and discuss our problem setting that extends standard autonomous RL to the multi-task setting, where offline datasets from other tasks must be leveraged to improve performance.
\citet{sharma2021autonomous} formalize autonomous RL in terms of two MDPs: a non-episodic training MDP, $\mathcal{M}_T$, where the environment resets only occasionally or never at all,
%%SL.1.28: maybe we can elaborate?
and the corresponding episodic evaluation MDP $\mathcal{M}$, where the agent must successfully perform the task from initial states sampled from $\rho(s)$. The transition dynamics $P$ and the reward function $r$ are the same in the two MDPs. The agent must learn to perform the task in $\mathcal{M}_T$, but will be evaluated in terms of its performance on $\mathcal{M}$. Since only infrequent resets are allowed during training in $\mathcal{M}_T$, simply maximizing the original reward $r(\bs, \ba)$ in $\mathcal{M}_T$ may not lead to the best performance on $\mathcal{M}$~\citep{sharma2021autonomous}, and so the agent must learn to reset itself while training so that it can learn to attain good performance from the initial states it will encounter at test-time in $\mathcal{M}$.

%\textcolor{red}{Write the optimization objective for autonomous RL?}

% This can be formalized as follows:

% \begin{align}
%     \max_{\pi}~~~& J_\text{standard}(\pi) \\
%     &~\text{s.t.}~~ \pi \leftarrow \mathbb{E}
% \end{align}

%%AK: maybe add a transition line here....
\textbf{Offline reinforcement learning via AWAC.} In this paper, we utilize an offline RL method, advantage-weighted actor critic (AWAC)~\citep{nair2020accelerating}, to extract skills from prior data. AWAC is an actor-critic method that alternates between a policy evaluation phase (Equation~\ref{eqn:awac_update}), where it trains a parameteric Q-function, $Q_\phi(\bs, \ba)$, to minimize the error between two sides of the Bellman equation on the samples from the offline dataset, and a policy improvement phase (Equation~\ref{eqn:awac_actor_update}) where it improves a parametric policy $\pi_\theta(\ba|\bs)$ via advantage-weighted updates. Advantage-weighted updates perform policy improvement by cloning actions that are highly advantageous under the learned Q-function and are hence, more likely to improve upon the data-collection policy. Denoting the offline dataset as $\mathcal{D} = \{(\bs_i, \ba_i, \bs'_i, r_i)\}_{i=1}^N$, where $(\bs_i, \ba_i, \bs'_i, r_i)$ denotes a single transition, the training objectives for AWAC are given by:
\begin{align}
\label{eqn:awac_update}
\widehat{Q}^\pi_\phi \leftarrow &\arg\min_\phi~ \mathbb{E}_{\bs, \ba, \bs' \sim \mathcal{D}}\left[(Q_\phi(\bs, \ba) - (r + \gamma Q_\phi(\bs', \ba')))^2\right]\\
\widehat{\pi} \leftarrow & \arg\max_\theta~ \mathbb{E}_{\bs, \ba \sim \mathcal{D}} \left[ \log \pi_\theta(\ba|\bs) \cdot \exp(\widehat{A}^\pi(\bs, \ba)) \right], \nonumber\\
\text{~where~~~} & \widehat{A}^\pi(\bs, \ba) := \widehat{Q}^\pi_\phi(\bs, \ba) - \mathbb{E}_{\ba' \sim \pi}\left[\widehat{Q}^\pi_\phi(\bs, \ba')\right]. \label{eqn:awac_actor_update}
\end{align}
% We will now present our robotic system, which allows us to solve a variety of challenges in robot learning together by simply leveraging prior interaction datasets.

% \textcolor{red}{move to methods: since this is how \textbf{we} do it} Additionally, we augment the reward function in the training MDP to incentivize the agent to reset the environment to the initial state distribution after performing the task. In the training MDP, the agent receives reward $r_f(s, a)$ while attempting to perform the task. After successfully completing the task the agent recieves reward $r_b(s, a)$ for returning the environment to the initial state distribution. In the evaluation MDP, the agent only recieves reward $r(s, a) = r_f(s, a)$, since the environment is reset after every episode. 


%%SL.1.17: My sense is that it's a good idea to have a section that goes over basic (boring) boilerplate definitions and stuff like that. Basically, how do we define MDP etc. At the same time, we also need a paragraph or two somewhere that defines the problem statement. That doesn't necessarily go into this section (in fact, perhaps it would be best if it doesn't), but it's important to have it somewhere, so that it's clear to the reader what assumptions we make and what problem we are tackling. For the problem definition I agree that it could go somewhere else (e.g., into our methods section).



==> rss/text/4-method.tex <==
\section{Problem Statement}
\label{sec:problem_statement}
In this section, we will formalize our problem statement and describe our evaluation setup. Our goal is to utilize data from previous tasks to address three key challenges in robotic reinforcement learning: sample-efficiency, autonomous learning and generalization and robustness to unseen test conditions, all together. To this end, we assume access to a prior dataset $\mathcal{D}_\text{prior}$ of experience collected from a multiple training tasks, $\Pi = \{\tau_1, \tau_2, \cdots, \tau_N\}$:
\begin{align}
    \label{eqn:dataset_equation}
    \mathcal{D}_\text{prior} = \cup_{j=1}^N \mathcal{D}_j; ~~~ \mathcal{D}_j = \left\{ \left(\bs^j_i, \ba^j_i, \bs'^j_i, r^j_i\right) \right\}_{i=1}^K,
\end{align}
where $\mathcal{D}_{j}$ denotes the chunk of the prior data corresponding to task $\tau_j$. Our goal will be to extract a rich repertoire of skills from this diverse, multi-task prior dataset, $\mathcal{D}_\text{prior}$, and use them to quick solve a new target task $\taustar$ that was not seen in training, i.e., $\taustar \notin \Pi$. 
%%AK: feel free to change notation, it is defined in defs.tex
Additionally, we require that this new task must be solved with minimal resets: when the robot is practicing on the target task $\taustar$,
%%AK: is finetuning the right word here? or are we calling it something else?
it will only be infrequently provided with external resets, in accordance with the autonomous RL paradigm.
%%AK: maybe cite section prelims here
The learned agent is then evaluated on the same task $\taustar$, but this time it gets reset after every episode.

%%AK: might want to say something about generalization too



% define autonomous RL
% define that this setting corresponds to 


\section{
Autonomous Robotic Reinforcement Learning with Prior Data 
}
\label{sec:method}
% We now describe our method for leveraging data from previous tasks to address key challenges in robotic reinforcement learning: sample-efficiency, non-episodic learning, and generalization. We assume access to a dataset $\mathcal{D}$ of logged interactions from previous tasks, and 

We will now present our approach for leveraging data from previous tasks to address key challenges in robotic reinforcement learning: sample-efficiency, non-episodic learning, and generalization. Our system is designed to extract knowledge from $\mathcal{D}_\text{prior}$ that enables learning new tasks more efficiently, with fewer resets, and in a way that results in broader generalization to variations in the environment.

Our method, which we call Autonomous RobotIc REinforcement Learning (\methodName), consists of two phases (see Figure \ref{fig:overview}). First, we extract useful skills and representations from $\mathcal{D}_\text{prior}$ using offline reinforcement learning, as discussed in Section~\ref{sec:offline}. This essentially provides our method with the ``prior knowledge'' that it will use to then perform near-autonomous training for new tasks. 
%%AK: is it obvious that we use a reset controller at this stage? 
% We use this prior knowledge to initialize both a task and \doubt{reset controller for a new task}, as discussed in Section~\ref{sec:online}, enabling learning with only occasional manual resets. 
We use this prior knowledge to both quickly learn the new task, and to bootstrap a separate policy that resets the environment back to an initial state, so that the agent can continue practicing without the need for external resets after every attempt. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/fig1_v0.pdf}
%     \caption{\textbf{Overview of our system.} In the offline stage (left), we train a multi-task policy that captures prior knowledge from an offline dataset of previously experienced tasks. Then, in the online stage (right), this multi-task policy is used to initialize learning for a new task, providing both a forward policy and a backward (reset) skill, and improving learning speed and generalization. We demonstrate that this approach leads to sample-efficient learning of generalizable policies with a significant reduction in the need for manual interventions (i.e., resets).}
%     \label{fig:overview}
%     %%SL.1.28: I think this figure structurally has the right idea, but I think it's missing the notion of pretraining. Right now, it kind of just looks like both prior data and new task data is merged into a single buffer that is used to train a policy, but in fact there is also a pretraining phase. The diagram also doesn't clearly show that there are two policies -- a forward and a backward policy. Aesthetically, I might also recommend the trying to make the pictures of the robots bigger so that it's clearer what is going on, and try to show different tasks if possible.
% \end{figure}

\subsection{Learning From Prior Data with Offline RL}
\label{sec:offline}
Given a dataset from previous tasks, we first aim to extract skills and representations that could be useful for learning downstream tasks. The multi-task dataset $\mathcal{D}_\text{prior}$ can come from many different sources: human demonstrations, sub-optimal data from previous reinforcement learning experiments, or even data collected using (imperfect) hand-engineered policies. We assume that the tasks in this dataset are structurally similar to the new tasks we wish to learn, so a (multi-task) RL agent that has been trained on this dataset should explore new environments much more effectively than a randomly initialized policy. For example, the prior data might of consist picking and placing a variety of objects under a wide variety of lighting conditions and backgrounds. An agent that successfully learns the skill of picking and placing from this prior data would then be well-prepared to learn how to pick up a previously unseen object, and place it in a previously unseen container.
%%AS.1.27 Not sure if need this next line, so I commented it out for now. 
% Thus, we want to obtain the optimal policy $\pi$ and value function $\mathcal{Q}_\phi$ for the tasks in the prior data, motivating the use of an offline RL algorithm.

%%AS.1.27 Commented out the next two lines to reduce redundancy (if we want to add them back in, we'll have to cleanup a little)
% Since a new task task may be similar to any one of the tasks in the prior data, we want to use offline RL to learn a policy and value function capable of performing each task. 
% Then, we can solve the new task quickly by adapting the policy and value function, potentially interpolating between the prior tasks. 
% We assume the prior dataset $\mathcal{D}$ is partitioned into individual task datasets, such that $\mathcal{D} = \cup_{i=1}^N \mathcal{D}_i$, each composed of transitions, such that $\mathcal{D}_i = \{(s_j, a_j, s'_j, r_j)\}_{j=1}^N$. 
The provided prior dataset $\mathcal{D}_\text{prior}$ is partitioned into individual task datasets (Equation~\ref{eqn:dataset_equation}), {and to make use of this multi-task dataset for downstream tasks, we train a conditional policy $\pi_\theta(\ba | \bs, \bz)$ using offline RL.} This policy is conditioned on a task index $\bz$ (represented as a one-hot vector) that informs the agent which task it is performing. Conditioning on task indices is a common strategy while training multi-task policies~\cite{kalashnikov2021mt}. Training a single multi-task policy offers several advantages over training separate policies on the prior dataset. First, we are able to learn a representation of policy inputs and outputs (in this case, images and desired change in end-effector pose, respectively) which is shared across tasks, and is therefore more likely to generalize well when faced with new inputs: both through interpolation (if the new task is similar to previously seen tasks), and extrapolation (for novel tasks). 
Second, when attempting a new task, we only need to sample actions from a single pre-trained policy, as opposed to choosing from an ensemble of pre-trained policies.
Finally, this also allows our method to gracefully scale with the number of tasks in the prior dataset. 
% Na\"{i}vely optimizing a single policy $\pi(a | s)$ and value function $\mathcal{Q}_\phi(s, a)$ to perform all the tasks often fails due to gradient interference so, as is typical in multi-task RL, we learn a policy $\pi_\theta(a | s, z)$ and value function $\mathcal{Q}_\phi(s, a , z)$ conditioned on a task index $z$ that informs the agent which task it is performing. 
% In practice, we augment the observations from a given task with the one-hot task index vector for that task. 
After the offline learning phase, we have a multi-task policy $\pi_\theta(\ba | \bs, \bz)$ that can perform each of the tasks in the prior data. % and value function $\mathcal{Q}_\phi(s, a, z)$
In Section \ref{sec:setup} we discuss the specific tasks we use in our prior data and how we generate the prior dataset for our experiments.

\subsection{Autonomous Online Training}
\label{sec:finetuning}
The main goal of our system is to enable the robot to efficiently learn a new task with minimal externally provided environment resets, leveraging the prior knowledge distilled into the offline multi-task policy discussed in the previous section. Since the environment is not frequently reset, the agent must simultaneously learn to perform the task and reset the environment to the initial state so it can continue practicing. Prior work has tackled this problem by learning distinct forward and backward controllers, alternating between applying the forward controller to perform the task and applying the backward controller to reset the task \cite{han2015learning, eysenbach2017leave, zhu2020ingredients, xu2020continual, sharma2021autonomoussubgoal}. We adopt an analogous strategy, but we leverage the multi-task policy described in the previous section to bootstrap learning in both the forward and backward direction, which both helps to overcome the exploration challenge and provide automated resets more quickly than if the backward controller were trained from scratch.

To enable this, we fine-tune the parameters of the policy $\pi_\theta(\ba | \bs, \bz)$ obtained after the offline phase with online data from the new task $\taustar$, that we denote as $\mathcal{D}_{\taustar}$, similar to prior work that uses online fine-tuning to improve upon policies learned via offline RL alone~\cite{nair2020accelerating}. 
However, since we have a multi-task policy, we must confront the question of which skill(s), parameterized by task indices $\bz$, should be chosen to start finetuning for the forward and backward controller.
In order to automatically determine which prior skill (or combination of prior skills) to finetune, we treat the task index $\bz$ as a continuous, learnable parameter and use data collected during online reinforcement learning to select the $\bz$’s best suited for the given new task. 
In this sense, we treat $\bz$ as a task embedding~\cite{hausman2018learning} that is automatically adapted for the task at hand, similar to prior work in meta-reinforcement learning~\cite{rakelly2019efficient}.

Since we aim to learn both a forward and backward controller, we optimize for two skills, parameterized by two distinct task embeddings $\bz_f$ and $\bz_b$, that respectively perform the task and reset the environment. 
Conditioning the policy on $\bz_f$ results in the forward controller $\pi_\theta(\ba | \bs , \bz_f)$ that performs the task, whereas conditioning the policy on $\bz_b$ results in the backward controller $\pi_\theta(\ba | \bs, \bz_b)$ that resets the environment according to the initial state distribution of the task $\taustar$. During fine-tuning we alternate between applying the forward controller and backward controller, optimizing the forward controller with rewards for completing the task $r_f(\bs, \ba)$ and the backward controller with rewards for returning to the initial state distribution $r_b(\bs, \ba)$.
We optimize the parameters $\bz_f$ and $\bz_r$ in tandem with the policy and value function parameters $\theta$ and $\phi$. The parameters of the policy and value function are updated using using an actor-critic algorithm; we utilize the AWAC~\citep{nair2020accelerating} algorithm in our experiments. The embeddings $\bz_f$ and $\bz_r$ are optimized differently, as we discuss next.
% After fine-tuning, we have two task embeddings, $\bz_f$ and $\bz_b$ that induce a forward controller $\pi_\theta(\ba | \bs , \bz_f)$ and backward controller $\pi_\theta(\ba | \bs, \bz_b)$.
%%AK: notation mistmatch above

% HW.1.26 Re the below comment: in reality there is only one policy. You get the forward policy by conditioning on the forward task embedding z_f and the backward policy by conditioning on the backward task embedding z_b. I attempted to make this more clear above.
%%SL.1.26: Can we refine the above paragraph to explicitly introduce terminology (symbols) for the forward and backward policy?
\textbf{Optimizing task embeddings $\bz_f$ and $\bz_b$.} Since our goal is to learn on the target task $\tau^*$ as quickly as possible, and with minimal resets, we need to effectively explore the environment during online training. An ideal approach that explores effectively must not prematurely commit to a particular value of $\bz_f$ and $\bz_b$ until the online experience clearly indicates so, and at the same time, it should be fast at collapsing to the correct values of $\bz_f$ and $\bz_b$, when it is very much apparent from the online experience gathered till then. While one straightforward approach to optimize $\bz_f$ and $\bz_b$ is to simply treat them as additional parameters and update them via gradient descent, however this requires initializing $\bz_f$ and $\bz_b$ to an initial guess, which means that only these randomly chosen skills will be fine-tuned. Furthermore, the \emph{local} nature of gradient updates may simply inhibit fast adaptation of these embeddings. 

Instead, we found that the cross-entropy method (CEM)~\citep{??}
%%AK: cite CEM here
provided us with a favorable balance between exploration and exploitation. CEM provides a way to initialize the task embedding to a \emph{distribution}, which ensures that we do not have to commit to fine-tuning any one particular skill. How is this CEM procedure performed? Since we want to optimize both the forward and backward embeddings $\bz_f$ and $\bz_b$, we fit two sampling distributions with CEM, $q_f(\bz)$ and $q_b(\bz)$. The distribution of tasks in the prior data $\mathcal{D}_\text{prior}$ provides us with a natural (and hopefully informative) prior to initialize $q_f(\bz)$ and $q_b(\bz)$. On each iteration of training,
we sample a $\bz$ from either $q_f(\bz)$ or $q_b(\bz)$ and roll out the policy conditioned on this $\bz$ value for $M$ steps. These $M$-step trajectories would essentially correspond to an episode in episodic RL, however the environment is (typically) not reset
%%SL.1.28: not always reset? maybe add a footnote to say we actually reset [with some freq]
%%AK: since this info is there right after this, perhaps we don't need it? But open to adding a footnote
afterward. We alternate between sampling the $\bz$ from $q_f(\bz)$ or $q_b(\bz)$ to alternate between applying the forward and reset controllers. The reward function correspondingly alternates between $r_f(\bs, \ba)$ and $r_b(\bs, \ba)$. We periodically
re% maybe introduce another letter here to denote what periodically means
fit $q_f(\bz)$ and $q_b(\bz)$ to the $J$ most recently sampled $\bz$'s that resulted in trajectories that successfully completed or reset the task, respectively. We update the policy and value function parameters $\theta$ and $\phi$ using the update steps from an RL algorithm as summarized in Algorithm~\ref{alg:method}.
%%SL.1.28: summarized in Algorith XX
Every $N$ steps, we provide an external reset to the environment. However, $N >> M$, so the external resets are infrequent. For example, in one of our real world tasks, $M=20$, and $N=400$.
%%SL.1.28: in our implement, N is ?? and M is ??
In theory, we could run our method without any manual resets at all, but we found a small number of manual resets necessary to recover from certain states, similarly to prior work in the area~\cite{eysenbach2017leave}. 


% we wish to optimize $\bz_f$ and $\bz_b$ using a more global for the target task  
% Since we want to optimize a forward and backward task embedding, $\bz_f$ and $\bz_b$, we fit two sampling distributions with CEM, $q_f(\bz)$ and $q_b(\bz)$. We initialize both distributions by fitting them to the prior distribution of task indices observed in $\mathcal{D}_\text{prior}$ used for offline training.
% used during the offline learning phase, since the behaviors in the offline data are likely to result in good initial exploration on the new task.
%%SL.1.28: I think there is a simpler explanation -- if we fit it to the training data, then we literally initialize it to the prior distribution, maybe we just say that?
% We then refine $q_f(z)$, $q_b(z)$, and the policy and value function parameters $\theta$ and $\phi$ with online data. To do this,
% %%SL.1.28: on each iteration of training
% we sample a $z$ from either $q_f(z)$ or $q_b(z)$ and roll out the policy conditioned on this $z$ for $M$ steps. These $M$-step trajectories correspond to an episode in episodic RL, however the environment is not reset
% %%SL.1.28: not always reset? maybe add a footnote to say we actually reset [with some freq]
% afterward. We alternate between sampling the $z$ from $q_f(z)$ or $q_b(z)$ to alternate between applying the forward and reset controller. The reward function correspondingly alternates between $r_f(s, a)$ and $r_b(s, a)$. We periodically
% re% maybe introduce another letter here to denote what periodically means
% fit $q_f(z)$ and $q_b(z)$ to the $J$ most recently sampled $z$'s that resulted in trajectories that successfully completed or reset the task, respectively. We update the policy and value function parameters $\theta$ and $\phi$ using the update steps from an RL algorithm.
% %%SL.1.28: summarized in Algorith XX
% Every $N$ steps, we provide an external reset to the environment. However, $N >> M$, so the external resets are infrequent.
% %%SL.1.28: in our implement, N is ?? and M is ??
% In theory, we could run our method without any manual resets at all, but we found a small number of manual resets necessary to recover from certain states, similarly to prior work in the area~\cite{eysenbach2017leave}. 

%%SL.1.28: I feel like we have a somewhat tortured organization here, because we are trying to explain CEM first and then say why. Perhaps we should simply switch the order of the next two paragraphs, first explaining optimizing task embeddings and then the CEM stuff? In some sense we should be able to explain optimizing zf and zb largely independently of how we do it, and motivate the q(z) thing from the standpoint of exploration or something? (and then oh it's so convenient that CEM basically does this)


\iffalse
\textbf{Cross-Entropy Method (CEM).} We use a gradient-based actor-critic algorithm to optimize the policy and value function parameters using the online data. However, we use the cross-entropy method (CEM) to optimize the task embeddings. 
We defer our reasoning for choosing CEM until after explaining our application of CEM. 
The cross entropy method is a Monte-Carlo optimization procedure that iteratively refines a sampling distribution $q(z)$ in order to maximize an expectation $\mathop{\mathbb{E}}\left[\mathcal{R}(z)\right]$. 
The sampling distribution $q(z)$ can be initialized to a simple distribution, such as a mixture of Gaussians.
CEM consists of two steps.
First, CEM samples a series of points $z_1, ..., z_n$ from $q(z)$. 
Then, the method evaluates the objective function on these points and updates $q(z)$ to fit to the $J$ points with the most optimal objective values, where $J$ is a hyperparameter (a positive integer that is smaller than total number of evaluations conducted). Alternating between these two steps narrows the sampling distribution to the region of the domain with the optimal objective values.
%SL.1.28: definitely put this later, if we're out of space could even put it in an appendix
%%AK: if what I wrote above seems reasonable, we shouldn't need this para. We can move this para to an appendix.
\fi


% Here I'm explaining the main reason I think CEM makes sense here: we can easily initialize the CEM models with the one-hot train task indices. Is there another more fundamental reason? -HW
%%AS.1.27: I guess the argument here is that you can initialize z with a distribution instead of a (fixed) vector. I re-worded this paragraph, but I am still unsure if it would be clear to a (new) reader, so further edits here can be useful. 
% In principle, we could optimize the task embeddings jointly with the policy (and value function) parameters using RL. However, we found that CEM has a particular advantage in this setting. CEM provides a way to initialize the task embedding to a \emph{distribution}, as opposed to gradient-based optimization which would require initializing the task-embedding to a fixed vector, and then performing local gradient steps around it. Using CEM allows us to effectively conduct multi-modal exploration in a new environment, and ensures we don't commit to fine-tuning any one specific skill without having conducted any exploration in the new environment. 
%for intelligently initializing the task embedding optimization procedure by initially fitting $q_f(z)$ and $q_b(z)$ to the one-hot task indices used during offline learning. Initially conditioning the policy on embeddings close to the task indices used in offline learning bootstraps exploration since the task indices induce behaviors similar to those in the prior data, which may succeed on the new task with non-negligible probability. CEM then exploits these successes to narrow the search to the regions of the embedding space that optimally perform or reset the new task. 

\subsection{Algorithm Summary}
To summarize, we first perform offline learning on the provided dataset $\mathcal{D}_\text{prior}$ (see Algorithm~\ref{alg:offline}). We use offline RL to obtain a multi-task policy $\pi_\theta(\ba | \bs, \bz)$ and value function ${Q}_\phi(\bs, \ba, \bz)$. Then, in the online phase (see Algorithm~\ref{alg:online}), we adapt this policy and value function to a new task. Notably, the offline phase occurs only once, but the online phase can be run many times to efficiently learn many new tasks. Online adaptation begins by fitting two CEM sampling distributions, $q_f(\bz)$ and $q_b(\bz)$, which are initialized to the distribution of task indices seen during offline learning. Then, we collect data for the new task by sampling a task embedding $\bz$ from a CEM model and rolling out the policy conditioned on this $\bz$ for $M$ steps. If the trajectory obtains reward for completing or resetting the task, we switch to sampling from the opposite CEM model. This corresponds to alternating between applying a forward and backward controller. We use the online data to refine the sampling distributions $q_f(\bz)$ and $q_b(\bz)$ with CEM and the policy and value function with RL. Every $N$ steps we manually reset the environment, sampling a state from the initial state distribution $s \sim \rho(s_0)$. Our system allows us to learn the new task efficiently and with minimal environment resets by leveraging prior data from previous tasks.
%%SL.1.26: I would suggest making this paragraph more detailed and really walk through Algorithm 1 line by line.


\begin{algorithm}[]
    \newcommand{\MYCOMMENT}[1]{~\textcolor{gray}{// #1}}
    \textbf{Input:} offline dataset $\mathcal{D}_\text{prior}$
    \begin{algorithmic}
        \STATE Initialize policy $\pi_\theta(\ba|\bs,\bz)$, value function ${Q}_\phi^\pi(\bs, \ba, \bz)$
        \STATE $\pi_\theta(\ba|\bs,\bz), {Q}_\phi^\pi(\bs, \ba, \bz) \gets$ \texttt{OfflineRL}($\mathcal{D}_\text{prior}$)
    \end{algorithmic}
    \caption{
    \methodName~offline phase
    }
    \label{alg:offline}
    \label{alg:method}
\end{algorithm}
%%SL.1.28: try to arrange this so that Alg 1 and Alg 2 are right next to each other (eg one above the other) on the same page

\begin{algorithm}[]
    \newcommand{\MYCOMMENT}[1]{~\textcolor{gray}{// #1}}
    \textbf{Input:} pre-trained policy $\pi_\theta(\ba|\bs,\bz)$ and value function ${Q}_\phi^\pi(\bs, \ba, \bz)$
    \begin{algorithmic}[1]
        
        \STATE Initialize buffer $\mathcal{B}$, CEM models $q_{f}, q_{r}$
        \STATE Fit $q_f(\bz)$ and $q_b(\bz)$ to offline task indices
        \STATE $d \gets f$ \MYCOMMENT{task direction, f is forward, b is backward}
        \WHILE{\NOT done}
            \STATE $s \sim {\rho(\bs_0)}$ \MYCOMMENT{sample initial state (i.e external reset)}
            \FOR{$N$ steps}
                \STATE \MYCOMMENT{sample new task embedding if you reach max episode length}
                \IF{steps \% $M == 0$} 
                    \STATE $\bz \sim q_d$ % \doubt{what is $q_d$?} %\MYCOMMENT{sample task embedding} 
                \ENDIF
                \STATE Sample $\ba \sim \pi(\cdot | \bs, \bz)$, observe $\bs' \sim p(\cdot|\bs, \ba)$
                \STATE $\mathcal{B} \gets \mathcal{B} \cup \{(\bs, \ba, {r}_d(\bs', \ba), \bs', \bz\}$
                \IF{${r}_d(\bs', \ba)$}
                    \STATE \texttt{switch}$(d)$ \MYCOMMENT{switch task direction}
                \ENDIF
                \STATE update $\pi_\theta, {Q}_\phi^\pi$ with RL
                \STATE update $q_f(\bz), q_b(\bz)$ with CEM
                \STATE $\bs \gets \bs'$
            \ENDFOR
        \ENDWHILE
    \end{algorithmic}
    \caption{
    \methodName~online adaptation
    }
        \label{alg:online}

    \label{alg:method}
\end{algorithm}



\subsection{Implementation Details}
We choose advantage-weighted actor-critic (AWAC) as the underlying RL algorithm for both the offline and online phase because it addresses the specific challenges that arise when learning behaviors offline and then finetuning them online \cite{nair2020accelerating}. We present a technical description of AWAC in Section~\ref{sec:prelims} and provide the specific hyperparameters that we use in our experiments in the Appendix. 
% do we actually need to explain AWAC here? maybe not -HW
%%AK: I dont think so, so I moved this to the prelims 
% A central challenge in offline RL is correcting for errors due to distribution shift between the offline data and data collected at test time. Offline RL algorithms often address this distribution shift by constraining the learned policy to stay close to an explicit behavior model of the data seen so far. However, this leads to slow online finetuning since it is difficult to update the a model of the behavior policy online. AWAC addresses this challenge by avoiding modeling the behavior policy explicitly and instead implicitly constraining the learned policy to stay close to the data seen so far. We provide the specific hyperparameters for AWAC in the Appendix. 
% this is arguably an important method detail rather than implementation detail and could go earlier -HW
Notably, since AWAC is an off-policy RL algorithm, we have the option of continuing to train on the prior data during the online phase. We hypothesize that including the prior data during online adaptation prevents the agent from overfitting to the new task and improves generalization, so we continue to train on the prior data even during the online fine-tuning phase. 
%\doubt{We include prior data in the online phase for our evaluations since generalization is essential.}
%%AK: this probably needs to be explained. Why didnt we include it in simulation?

As our goal is to make robotic learning as autonomous as possible, we use images observations as part of our input to the RL agent. Image observations allow our system to learn from a diverse range of different tasks without needing to hand-engineer state representations suitable for each task. Because we are learning from images we use convolutional neural networks to model the policy and Q-function (see Figure \ref{fig:arch}). 
We provide the specific architecture in the Appendix. 
The observations additionally consist of the state of the robot's joints, and the task embedding $\bz$. We use a Gaussian mixture model as the sampling distribution for CEM.
% should we reveal that we set the number of components of the GMM equal to the number of tasks here, thereby preventing CEM from finding continuous embeddings, or save this for later?
%%AK: that's a detail for later I think. 
For our evaluations in simulation we fit the CEM sampling distributions to the $J=25$ most recent successful embeddings. 
%\doubt{once every 10 trajectories}. 
%%AK: how do you define trajectories here? I see the intent, but it might be confusing to a reader
%%AS: commented this one detail out for now, can add in appendix or something. 
For our evaluations in the real world, we fit the CEM models to the $J=10$ most recent successful embeddings. 
% every 10 trajectories. 

% could stick this in the appendix
\begin{figure}[!h]
    \centering
    \vspace{-0.05in}
    \includegraphics[scale=0.23]{figures/convnet.png}
    \vspace{-0.1in}
    \caption{\textbf{CNN architecture we use for our policy.} Our method learns robotic manipulation skills from raw image inputs, and fine-tunes to new skills with minimal resets while leveraging prior experience. %we should make this figure not specific to the policy since policy and q function use the same conv net architecture
    }
    \label{fig:arch}
    \vspace{-0.15in}
\end{figure}



==> rss/text/5-experiment-setup.tex <==
\section{Experiment Setup}
\label{sec:setup}

We now describe the system and experiment setup in our evaluation, as well as the data collection and training process.

%%SL.1.28: it would be really good to put a wrapfigure picture of the robot into this paragraph
\textbf{Robotic platform.}
We evaluate our approach using a 6-DoF WidowX robotic arm. The 7D action space of the system consists of 6D Cartesian end-effector motion, corresponding to relative changes in pose, as well as one dimension to control the opening and closing of the parallel jaw gripper. The state observations consist of the joint angles and RGB images from an overhead camera, which are 48$\times$48 in simulation and 64$\times$64 in the real world.
%The robotic platform we use is a 6-DoF WidowX robotic arm. The action space is 7-dimensional and consists of three values representing the change (delta) in the end-effector's Cartesian coordinates, three values representing the change in its orientation, and one dimension for actuating the gripper. The observations passed to \methodName\ consist of a camera image and the robot joint angles. We use 48$\times$48 RGB images in simulation and 64$\times$64 RGB images in the real world. The state of the robot is a 6D vector of the joint angles. We study two classes of manipulation tasks, discussed below, and for each class construct different tasks with different objects and containers.
%%Ak: the stuff below is a nitpick, but is it the *objective* for the algorithm (as in you evaluate the robot on this metric, and do we evaluate the backward controller at all?) or is it just the learning objective that we use?

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/real_world_objects.png}
    \caption{\textbf{Objects used to construct the container placing tasks in our experiments.} The upper part of the figure shows containers and objects used in the offline data for pretraining, the lower part shows test objects that are used as part of new tasks for online training.}
    \label{fig:containers}
    \vspace{-0.15in}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/robot_3_tasks_film_strip.jpg}
    \caption{Three downstream tasks on our real-world robotic setup. Each row shows snapshots from a single episode, from left to right. The top row depicts the drawer task, where the objective is to open the drawer, and place an object inside the drawer. The middle and bottom rows depict different container tasks, where the goal is pick an object from the workspace, and place it either on a plate, or inside a pot, depending on the task.}
    \label{fig:downstream_tasks}
    \vspace{-0.2in}
\end{figure}

\textbf{Evaluation tasks.} The tasks, some of which are shown in Fig.~\ref{fig:downstream_tasks}, involve interacting with objects and either containers or drawers, with each task corresponding to a different object and a different container. For container picking and placing tasks, there are 20 possible training objects and 4 possible training containers, including plates and cups (see Fig.~\ref{fig:containers}, and 2 unseen test objects and 2 unseen test containers. The prior data for the offline phase consists of 20 forward and 20 backward tasks with random object-container combinations. The simulated experiments have 16 possible objects and 1 container. For the drawer tasks, there are 4 possible training objects and 1 unseen test object, corresponding to 4 forward and 4 backward tasks. When a container is present, the tasks involve picking up an object from the table and placing it inside the container, whereas the drawer task additionally requires closing the drawer after inserting the object, and resetting requires opening the drawer and taking the object out. The new test tasks that we finetune in the online phase involve test objects that were not seen in training, but the same types of picking and placing behaviors. If indicated, the new task may also include a new type of container, as shown in Fig.~\ref{fig:containers}. All tasks have sparse rewards evaluated using a simple hand-designed vision system, with a reward of +1 if the robot completes the forward (or backward) task, and 0 otherwise. While such rewards are easy to define, they present a substantial challenge for RL.

%\noindent \textbf{Pick and place.} In this setting, the objective of the forward controller is to pick up an object from the workspace and place it on or inside another object. For example, the objective can be to pick up a spoon and place it on a plate. The backward task is similarly a pick and place task, but in the reverse direction, i.e. to pick up a spoon from the plate and return it to the workspace. 

%\noindent \textbf{Drawer.} In this setting the objective of the forward controller is to open the drawer, pick up the object from the workspace, and place it inside the drawer. The objective of the backward controller is to remove the object from the drawer, return it to the workspace and close the drawer. 

%\noindent \textbf{Reward functions.} Since our goal is to reduce human effort during robotic reinforcement learning as much as possible, the reward functions $r_f(\bs, \ba)$ and $r_b(\bs, \ba)$ we use to train our robots are sparse, and take on only binary values to minimize labelling effort.
% the Because our goal is make robotic reinforcement learning as autonomous as possible, in both settings the reward functions for the forward and backward controller, $r_f(\bs, \ba)$ and $r_b(\bs, \ba)$, are sparse. 
%The agent receives the +1 reward for successfully completing or resetting the task.

\textbf{Generating prior data.}
Our system can use prior data from any reasonable source, including demonstrations and prior RL runs, but for simplicity and consistency we employ a simple scripted policy to collect the prior data that we use for the offline phase. This provides a largely autonomous strategy to collect mediocre data for a variety of objects. While this scripted policy fails very frequently, offline RL can make use of such mediocre data effectively to pretrain value functions and policies for downstream fine-tuning. Since the prior dataset needs to provide an initialize for both the forward and backward directions for new tasks, we perform scripted collection in a reset-free manner, with the robot attempting to move the objects both into and out of containers. We collected about 500 trajectories for each of the 40 (20 forward, 20 backward) container pick and place tasks, and about 150 trajectories for each of the 8 (4+4) object/drawer tasks. All trajectories have a length of 30 time steps. The average success rates of the scripted policy were 0.38 for the simulated object-container tasks, 0.35 for the real-world object-container tasks, and 0.93 for the real-world object-drawer tasks.
%We use a scripted policy to generate the prior datasets for our evaluation. However, our system can use prior data from a variety of sources including demonstrations and data collected during previous reinforcement learning experiments. 
%Using scripted policies provides a (mostly) autonomous way to collect large datasets across a wide variety of objects.
%While our scripted policies do not exhibit high success rates, this is not a hindrance for our method since we can overcome these shortcomings during the online fine-tuning phase.  
%The goal of the prior dataset is to simply provide a strong initialization when learning new tasks. 
%We script policies to both perform and reset the tasks and collect data without manual resets, alternating between applying the forward and backward scripted policy. We collect data in this non-episodic manner to better match the distribution of data that we will later collect during non-episodic fine-tuning. 
%%AK: this sounds very procedural, as in "we do X, we do Y", maybe we can motivate first and then explain what we did. Otherwise it might be misinterpreted to say that our algorithm only works in some cases...? 
%%AS: Added some more details. 

%\noindent \textbf{For the pick and place setting}, tasks are distinguished by the choice of container and objects. To generate the prior dataset in the real-world, we collected data for 20 forward and 20 reverse tasks consisting of 20 different objects spanning 4 different containers. The scene for these tasks consisted of two objects and one container in varied positions. We collected approximately 500 trajectories of length 20 for each task. In the simulated setting, we collected data for 8 forward and 8 reverse tasks spanning 16 different objects and 1 container. 
%The scene for a container task in simulation consisted of 2 objects, 1 target object and 1 object to act as a distractor, as well as the container. 
%We collected 512 trajectories of length 30 for each task. The scripted policy for the container setting had an \doubt{average success rate of X in the real world and Y }. 

%\noindent \textbf{For the drawer setting}, tasks are distinguished by the choice of the object that is placed in the drawer. To generate the prior dataset, we collected data for 4 forward and 4 reverse tasks spanning 4 different objects. The initial scene for these tasks consisted of the object in varied locations and the drawer in a fixed location. We collected approximately 150 trajectories of length 30 for each task. The scripted policy for the drawer setting had an \doubt{average success rate of Y}.

\textbf{Online training setup.}
%\label{sec:finetuning}
Online training includes infrequent resets, to address the case where an object becomes stuck in a hard-to-reach (or unreachable) part of the workspace, but otherwise requires the robot to train autonomously. The resets are provided every 80 trials in simulation (about every hour), about every 20-30 trials (or about every 20-30 minutes) in the real world. Additionally, the pose of the robot is moved to a neutral position at the beginning of every trial, since there is no physical limitation that prevents doing this automatically, but the robot must still handle the fact that the objects in the scene maintain their position across trials.
%For the online phase of the pick and place tasks we collected trajectories of length 40 (i.e $M = 40$) in simulation and trajectories of length 20 in the real world. For the online phase of the real world drawer tasks we collected trajectories of length 35. At the end of a trajectory in the online phase we sample a new embedding from the CEM model and reset the robot to a neutral position. However, we do not reset the environment. In simulation, we provide an infrequent manual environment reset every 80 trajectories (i.e $N=3200$), corresponding to a reset every hour in the real world. For our real world pick and place tasks we provide a manual reset \doubt{every 30 trajectories, corresponding to Y minutes}. For our real world drawer task we provide a manual reset every 20 trajectories, corresponding to 20 minutes.

% \begin{figure}[!h]
%     \centering
%     \includegraphics[scale=0.2]{figures/task-images.png}
%     \caption{Images of the prior tasks and new tasks for the container and drawer setting in the real world and simulation.}
%     \label{fig:my_label}
% \end{figure}


\iffalse
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/tasks_18-20_film_strips.png}
    \caption{Three downstream tasks on our simulated robotic setup. Each row shows timesteps from a single test task, from left to right. For each of the tasks, the objective is to pick an object from the workspace, and place it into the container. The environments also have a ``distractor" object, so an indiscriminate grasping policy is unlikely to succeed, the policy must learn what object it needs to manipulate in the environment, as specified by the reward function.}
    \label{fig:my_label}
\end{figure}
\fi
%%SL: commenting out to save some space...

%%SL.1.26: My is that somewhere (perhaps after the algorithm summary) we need some kind of "Implementation Details" section that fully summarizes the implementation: what is the architecture (this is very important!), where are hyperparameters (maybe don't need this in main paper, but need to at least say where they can be found), etc. Basically all the details to make it reproducible. This is *very* important, missing such details is one of the most common reasons for robotics papers to get rejected. We might also want to have a "System Overview" section (e.g., a new top-level section) that explains the tasks, reward functions, etc. This is in the experiments section right now, but we could separate it into a "System" section vs a "Results" section


%%SL.1.17: is the stuff below still to be added? I think the stuff above is a good overview, but many details are missing -- we could put them into a separate "implementation details" section or something, but it's probably important to be more complete somewhere (potentially a different section); other details that may be good to include are: (i) the bit about how the data is collected (though this probably belongs in experiments); (ii) reward functions (same, could be in experiments); (iii) choice of RL method and motivation for why we used it; (iv) a long appendix with fully complete implementation details (robotics reviewers really love rejecting papers for being "non-reproducible"), including neural net architectures, learning rates, rewards, and all hyperparameters

==> rss/text/6-evaluation.tex <==
\section{Results}

\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/reset_free_2.pdf}
    \vspace{-1em}
    \caption{Experiments on simulated domains comparing our method to prior works in reset-free and multi-task learning. We see that ours is the only method that is able to learn in this limited-reset setting.}
    \label{fig:reset_free_graphs}
    
    \vspace{1em}

    \includegraphics[width=0.8\linewidth]{figures/sample_complexity_2.pdf}
    \vspace{-1em}
    \caption{Experiments in simulated domains comparing our method to learning without any prior data, and against an oracle approach which assumes access to offline dataset from the downstream task of interest. We see that our method adapts almost as quickly as the oracle approach, whereas reinforcement learning from scratch fails to make any progress. Note that this experiment is not in a limited-reset settings, resets were conducted at the end of every episode.}
    \label{fig:sample_efficiency_graphs}

\end{figure*}

Our experiments aim to evaluate the hypothesis that leveraging prior data from other tasks can simultaneously address multiple challenges in autonomous real-world robotic RL. To this end, we evaluate \methodName\ on a suite of simulated robotic manipulation tasks, and evaluate real-world online training with three new downstream tasks involving objects not seen in the prior offline data. Our goal is to answer the following questions: \textbf{(1)} Does leveraging prior data enable mostly autonomous learning of a new task in simulation and in the real-world? \textbf{(2)} How does \methodName\ compare to prior methods for leaning with minimal resets that do not use prior data? \textbf{(3)} Does leveraging prior data via \methodName\ lead to gains in sample-efficiency for a new task? and \textbf{(4)} Does \methodName\ produce policies that better generalize to new conditions?

Videos of the experiments can be found on the anonymous website: \url{https://sites.google.com/view/ariel-paper/}

\subsection{Evaluating \methodName\ in Simulation}
\label{sec:simulation}
We begin our empirical evaluation by comparing \methodName\ to prior approaches that also aim to tackle the challenges of autonomous learning or sample-efficient learning, in simulation. 

\subsubsection{\textbf{\methodName\ enables effective autonomous learning with minimal resets}} We compare to two prior approaches in our simulated experiments. To comparatively evaluate how well our method enables learning with minimal resets, we compare to the perturbation controller approach in \textbf{R3L}~\citep{zhu2020ingredients}, which alternates between training a forward controller to optimize a task-completion reward and training a perturbation controller that optimizes a novelty exploration bonus. This method has been proposed specifically to handle reset-free learning for real-world RL problems. We initialize the forward controller in R3L with the policy obtained by running offline multi-task RL on the prior data that used by our approach. We also compare to a method that does \emph{not} optimize the task embeddings $\bz_f$ and $\bz_b$ over the course of autonomous online fine-tuning. 
We refer to this approach as \textbf{Multi-task RL}. 
This is equivalent to first running multi-task offline RL on the prior dataset, and then fine-tuning the policy using a fixed task index (that was unused during pre-training) in an online phase afterwards. This method is conceptually similar to MT-Opt~\citep{kalashnikov2021mt}, but adapted to our pre-training and then fine-tuning setup, as opposed to the re-training from scratch approach followed by \citet{kalashnikov2021mt}. For instructive purposes, we also compare to an ``oracle'' version of our approach, labeled (\textbf{\methodName\ + resets}), which assumes access to external resets at the end of each episode. While resetting every episode is prohibitively expensive in the real-world, we can still run this method in simulation for our understanding.

%We first compare prior methods that aim to enable learning with minimal resets. Our primary point of comparison is \textbf{R3L} (\citet{zhu2020ingredients}), which alternates between training a forward controller to optimize a task-completion reward and training a perturbation controller that optimizes a novelty exploration bonus. In order to enable a fair comparison, we initialize the forward controller in R3L with the policy obtained by running offline multi-task RL on the prior data that used by our approach. 
% Then, during online training we label the data passed to the forward controller in R3L with an additional task index not used during the offline training. \doubt{can ths last line go in appendix?} 
%%AK: not sure what is the signfiicance of the above line for the results, maybe can go in the appendix as an implementation detail?.

%We also compare to a method that does \emph{not} optimize the task embeddings $\bz_f$ and $\bz_b$ over the course of autonomous online fine-tuning. 
%We refer to this approach as \textbf{Multi-task RL}. 
%This is equivalent to first running multi-task offline RL on the prior dataset, and then fine-tuning the policy using a fixed task index (that was unused during pre-training) in an online phase afterwards. 
%This method is closely related to how \citet{kalashnikov2021mt} learn new tasks in their multi-task setup, but adapted to our pre-training and then fine-tuning setup, as opposed to the re-training from scratch approach followed by \citet{kalashnikov2021mt}. 
% During online training, we label data collected by the forward and backward controller with two additional task indices that were unused in the offline phase. This ablation is similar to standard multi-task RL but with a distinct offline phase where some of the tasks are trained and an online phase where the rest of the tasks are trained.
%%AK: I am guessing the above line is not correct?

% For ablations, we compare to our method applied in the episodic setting (\textbf{ARIEL + resets}) where in the online phase we perform an external reset after every trajectory. We also compare to an ablation of our method without adaptation of the task embeddings (\textbf{Multi-task RL}). 
%We modify the policy and Q function architectures to accept two additional one-hot task indices. These task indices go unused during offline learning, 

The results in Figure \ref{fig:reset_free_graphs} show that \methodName\ is the only approach (and its oracle reset variant) are the only methods that succeed at learning the new tasks, and the full \methodName\ method closely matches final oracle performance. While the poor performance of prior methods might be surprising, recall that these tasks require using raw image observations and sparse 0/1 rewards, which present a significant challenge for any RL approach.
% likely due to the difficulty of learning from image observations and sparse rewards. 
While \textbf{R3L} and \textbf{Multi-Task RL} both succeeded at learning the tasks in the offline phase (see the Appendix for the offline RL learning curves), they are unable to make progress during online training of the new task. The comparison to \textbf{Multi-task RL} indicates the importance of adapting the task embeddings: if the task embeddings are not adapted to the new task, distributional shift in the task embeddings may severely hamper effective reset-free learning.
% \doubt{complete the conclusion of this experiment} 
Thus, we find that these methods cannot use skills learned offline to efficiently explore the new task. Our method solves this challenge with an explicit mechanism for searching in the space of task embeddings, starting from those used during offline learning, to induce substantially better-than-random initial exploratory behavior.


\subsubsection{\textbf{\methodName\ enables sample-efficient learning of the new task}}
% So far we have seen that \methodName\ is effective at enabling autonomous learning a new task, outperforming prior methods that provide technical solutions to this problem.
Next, we aim to evaluate whether our method, \methodName, enables better sample-efficiency than learning from scratch. To study the effect on sample complexity in isolation, we conduct experiments in which the environment is reset at the end of every episode (as opposed to the infrequent manual reset setting studied in the rest of this paper). We compare our method to simply applying RL to the target task, using the same RL algorithm as our system (\textbf{AWAC (no prior data)}). We also compare to an \textbf{oracle} method which is trained offline on data coming from only the single new task of interest and then trained online on the same task. Perhaps unsurprisingly, we found that learning from scratch fails in the challenging setting of learning from images and sparse rewards. However, our method learns just as efficiently as the oracle despite only having access to offline data for other tasks and not the new task of interest. Thus, our method demonstrates that properly leveraging prior data can improve sample-efficiency even when data is only available for other tasks.

\subsection{Real-World Experiments}
\label{sec:real_exps}

Next we evaluate the performance of \methodName\ when training online to solve new instances of the pick and place and drawer tasks, with previously unseen objects, in the real world. We aim to study how offline data can enable near-autonomous real-world RL with sparse rewards, and also study question \textbf{(4)}, understanding the effect that the prior data has on the generalization of the resulting policies. After pretraining on the datasets discussed in Section~\ref{sec:setup}, we evaluate \methodName\ by training three tasks that involve objects not seen in the prior data: placing a toy tiger in a drawer (which requires also closing the drawer, then opening it again to reset), placing a toy elephant in a pot, and placing a toy tiger on a lid. The pot, lid, elephant, and tiger were not seen in the prior data.  We evaluate success rates of the policy learned in the offline phase, the policy learned after 100 trials
%%AK; check this number
of online training, and the final policy after fine-tuning for 600 trials.
%%SL.1.28: can we replace the above by number of hours and trials (and also say what "final policy" takes...)

\subsubsection{\textbf{Autonomous fine-tuning with infrequent resets with \methodName\ significantly improves performance in the real world}} Observe in Tables \ref{tab:real-world-backward} and \ref{tab:real-world} that the performance of both the forward and backward controllers increases moderately after 100 trials (e.g., from 1/10 to 2/10 for the forward controller and from 1/10 to 8/10 for the backward controller on put elephant in pot) and substantially by the end of online training (e.g., from 2/10 to \textbf{7/10} for the forward controller and 8/10 to \textbf{10/10} for the backward controller) indicating that \methodName\ successfully optimizes the embeddings and policy parameters, with minimal resets, to perform the new task.  
% We include a plot of the success rate of the policy during fine-tuning in the Appendix. 
Since prior autonomous training methods did not make any learning progress in our simulated experiments, we did conduct additional real-world comparisons, but instead use the real-world setup to confirm that our method can enable real-world training, and then use it to study generalization as discussed below.

\subsubsection{\textbf{Training on diverse prior data improves zero-shot generalization in the real world}} In our final experiment, we aim to understand whether initializing from prior data provides \methodName\ with more robust representations that facilitate learning policies that generalize more effectively to new conditions with any further adaptation. In principle, if our only goal is to attain good performance on a single task, the best possible source of data should come from that task itself. But in the real world, we might often instead prefer a policy that is robust to variation in the task. In this case, we might hypothesize that the larger diversity present in the prior data might provide \methodName\ with representations that, even after online training on a single task, lead to better generalization.
%%SL: slightly rephrased this
%study if \methodName\ leads to the emergence of robust representations that allow the agent to generalize to new conditions, zero-shot, without any adaptation. In principle this must be possible: if \methodName\ can leverage the diversity of the prior data to learn a policy that generalizes, and utilize the autonomous online fine-tuning phase to correct inaccuracies in this generalizing policy, the resulting policy should be able to solve the task for a new condition, zero-shot. The ability to effectively extract generalizing skills from the offline data plays a crucial role in attaining any such zero-shot generalization ability. 

%To assess the zero-shot generalization capabilities of \methodName\, we first trained \methodName\ completely offline on the prior data from the pick and place and drawer settings described in Section~\ref{sec:setup}, then ran autonomous online fine-tuning on an intermediate task (object XX for the drawer setting and object YY for the pick and place setting), 

To study this hypothesis, we additionally evaluate the fine-tuned policies for the \emph{tiger in drawer} and \emph{tiger on lid} tasks in a setting where we swap out the object (but keep the same container). We do not expect the policies to succeed consistently in this case, but we see in Tables~\ref{tab:generalization1} and \ref{tab:generalization2} that the policies learned by \methodName\ exhibit some generalization, attaining an average success rate of \textbf{61.67\%} when evaluated at Epoch 15. We include a baseline that uses only the data for each online task (i.e., either only \emph{tiger in drawer} or only \emph{tiger on lid}) and no prior data. This baseline only succeeds in 26.67\% of trials on the new objects. This suggests that pretraining on prior data does effectively boost generalization.

%To assess the zero-shot generalization capabilities of \methodName\, we take the fine-tuned policies evaluated in Tables~\ref{tab:real-world} and~\ref{tab:real-world-backward}, and evaluate them towards solving the same task, but for new objects, without any adaptation. For comparison, we also trained a policy on the data gathered by \methodName\ during adaptation on a single downstream task, but this policy was not provided access to the prior data. 

%As shown in Tables~\ref{tab:generalization1} and \ref{tab:generalization2}, we find that the policy learned by \methodName\ exhibits much stronger zero-shot generalization abilities, solving the tasks with a success rate of \textbf{61.67\%} on average when evaluated at Epoch 15, compared to not using the offline prior data, which only succeeds 26.67\% times on average for the best training checkpoint. This implies that effectively utilizing prior offline data is crucial in generalizing to new settings, even when practice data from online adaptation can be provided for some setting.

Interestingly, we observe that while the success rate of \methodName\ during fine-tuning improves as more steps are performed (see 100 trials vs 600 trials in Tables~\ref{tab:generalization1} and ~\ref{tab:generalization2}), this also adversely affects the zero-shot generalization performance on a new object. This is to be expected, since even though our online training procedure replays the prior data, we train with a larger proportion of online data so with sufficient training we expect the policy to become more specialized to the fine-tuning task. 
% This is to be expected, since our online training procedure does not replay the prior data, so with sufficient training we expect the policy to forget its initialization. 
This observation is also consistent with prior RL works~\citep{cobbe2020leveraging,ghosh2021generalization} that note a drop in performance on test tasks as more updates are made on the training tasks. We anticipate the more principled early stopping or replay of the prior data could alleviate this issue, which is an interesting avenue for future work.

%This resembles a classic overfitting phenomenon and is not a fundamental problem specific to \methodName: many prior works in reinforcement learning~\citep{procgen_things} have noted such a drop in performance on a test task as more updates are performed on a training task and devising early stopping schemes
%%AK: while it is true that early stopping will fix this, I dont know of any thing to cite that has a solution for this early stopping. We could cite the workflow paper here, but it is not the same kind of overfiting...
%%AK: also add some numbers here, on train vs test from the tables here...
%can alleviate this degradation.

% one possible option -- detecting this overfitting and devising early stopping schemes will greatly mitigate the issue
% another option -- this opens up a 

% To assess if utilizing  



% \begin{figure*}
%     \centering
%     \begin{minipage}{0.4\textwidth}
%     \begin{tabular}{|p{1.5cm} | p{1.5cm}| p{1.5cm}| p{1.5cm}|}
%      \hline
%      & {Put Tiger in Drawer} & {Put Elephant in Pot} & {Put Tiger on Lid}\\
%     \hline
%      Offline only & 2/10 & 1/10 & 0/10\\ 
%     \hline
%      100 Trials & 4/10& 2/10 & 4/10\\
%      \hline
%      600 Trials & \textbf{9/10} & \textbf{7/10} & \textbf{7/10} \\
%      \hline
% \end{tabular}
%     \caption{Real-world evaluation of the forward controller in the container and drawer setting. Finetuning is mostly autonomous with a reset every 30 trials.}
%     \label{tab:real-world-backward}
%     \end{minipage}
% \end{figure*}


\begin{table}[]
    \centering
    \begin{tabular}{|p{1.5cm} | p{1.5cm}| p{1.5cm}| p{1.5cm}|}
     \hline
     & {Put Tiger in Drawer} & {Put Elephant in Pot} & {Put Tiger on Lid}\\
    \hline
     Offline only & 2/10 & 1/10 & 0/10\\ 
    \hline
     100 Trials & 4/10& 2/10 & 4/10\\
     \hline
     600 Trials & \textbf{9/10} & \textbf{7/10} & \textbf{7/10} \\
     \hline
\end{tabular}
    \caption{Real-world evaluation of the forward controller in the container and drawer setting. Finetuning is mostly autonomous with a reset every 30 trials.}
    \label{tab:real-world-backward}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{|p{1.5cm} | p{1.5cm}| p{1.5cm} |p{1.5cm}|}
     \hline
     & Put Tiger in Drawer & Put Elephant in Pot & Put Tiger on Lid\\
    \hline
     Offline Learning & 5/10 & 1/10 & 2/10\\ 
    \hline
     100 Trials & 6/10 & 8/10 & \textbf{6/10} \\
     \hline
     600 Trials & \textbf{7/10} & \textbf{10/10} & \textbf{6/10} \\
     \hline
\end{tabular}
    \caption{Real-world evaluation of the backward controller in the container and drawer setting. Finetuning is mostly autonomous with a reset every 20 trials.}
    \label{tab:real-world}
    \vspace{-0.5cm}
\end{table}


\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c ||c|}
        \hline
         & \multicolumn{3}{c||}{Our Method (\methodName)} &  \multicolumn{1}{c|}{No Prior Data} \\
        \hline
         Number of trials $\rightarrow$ & 100 & 360  & 600 & Best Epoch \\
        \hline
        Monkey & 5/10 & 6/10 & 5/10 & 6/10 \\
        Rabbit & 2/10 & 4/10 & 0/10 & 0/10 \\
        Hippo & 3/10 & 5/10 & 0/10 & 0/10  \\ \hline
        Tiger (fine-tuning) & 2/10 & 6/10 & 6/10 & 7/10 \\
        \hline
    \end{tabular}
    \caption{Generalization results, zero-shot performance on new task of picking several objects up and placing them in a container.}
    \label{tab:generalization1}
        \vspace{-0.5cm}

\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|c ||c|}
        \hline
         & \multicolumn{3}{c||}{Our Method (\methodName)} &  \multicolumn{1}{c|}{No Prior Data} \\
        \hline
         Number of trials $\rightarrow$ & 100  & 360  & 600 & Best Epoch \\
        \hline
        Pickle & 3/5 & 5/5 & 3/5 & 1/5 \\
        Turtle & 1/5 & 4/5 & 2/5 & 2/5  \\
        Dog & 2/5 & 2/5 & 4/5 & 2/5 \\ \hline
        Tiger (fine-tuning) & 3/5 & 3/5 & 3/5 & 1/5 \\
        \hline
    \end{tabular}
    \caption{Generalization results, zero-shot performance on opening a drawer and placing several objects.}
    \label{tab:generalization2}
    \vspace{-0.1cm}
\end{table}



%%%%%%%%%%%%%%%%%%%% OLD TEXT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse
In our empirical evaluations, we seek to show that leveraging prior data from previous tasks can solve key challenges in robotic learning, all combined together. To this end, we evaluate our approach \methodName\ on robotic manipulation tasks, in both real-world and in simulated domains with the goal of answering the following questions:
\begin{enumerate}
    % \item Does the system work in the real world?
    \item Does \methodName\ enable mostly autonomous learning of a new task?
    \item Does \methodName\ enable sample-efficient learning of a new task?
    \item Does \methodName\ produce policies that generalize to new conditions in the real world?
\end{enumerate}
We show that not only does our method outperform methods that learn from scratch, without using any prior data, in terms of both sample efficiency and generalization but it also outperforms other technical or algorithmic solutions for handling mostly autonomous learning proposed in prior work. We will discuss our results next, and we provide additional videos of our experiments on the anonymous website: \url{https://sites.google.com/view/ariel-paper/}.
%%SL.1.17: it would be good to more explicitly connect up these hypotheses to our claims earlier in the intro; a bit more motivation text prior to the list would be good, and it might be good to number the list so we can reference the numbers later


\subsection{Can \methodName\ learn effectively in the real-world?}
To validate if our full system is capable of actually learning to solve tasks even when faced with the challenges that arise in real-world scenarios, we evaluate \methodName\ on the both the pick and place and the drawer settings. Our goal is to check if \methodName\ can learn these tasks efficiently with minimal resets. First, we perform the offline phase of \methodName\ (Algorithm~\ref{alg:offline}) by training on prior data described in Section~\ref{sec:prior}, and then we perform online adaptation on a new task as outlined in Section~\ref{sec:finetuning}. For the drawer setting, the downstream task consists of manipulating a novel object, not seen previously the prior data. For the pick and place setting, the downstream task involves a scene that has both a new object and a new container, both not seen in the prior data. We evaluate the success rates of policy learned in the offline phase, the policy learned after 1 epoch (i.e. after conducting 400 environment steps and performing 1000 gradient steps on the actor and critic) of online adaptation, and the final policy after online adaptation.
% First we validate that our full system is capable of learning a new container placing and a new drawer task efficiently and with minimal resets in the real world. 
% We perform the offline phase by training on the prior data described in Section \ref{sec:prior}. Then, we perform online adaptation on a new task as outlined in Section \ref{sec:finetuning}. For the drawer setting, the new task consists of a new object, not seen the prior data. For the container setting, the new task consists of a new object and new container, both not seen in the prior data. We evaluate the success rate of policy learned in the offline phase, the policy learned after 1 epoch of online adaptation, and the final policy after online adaptation.
%Embeddings for the evaluation of the policy after offline learning are sampled from the prior distribution, i.e the task indices used during offline learning. After 1 epoch the task embeddings have mostly converged and by the end of online adaptation the task embeddings have fully converged. 
Observe in Tables \ref{tab:real-world} and \ref{tab:real-world-backward}, that performance of both the forward and backward controllers increases moderately after 1 epoch of training and substantially by the end of online training, indicating that leveraging prior data via \methodName\ to tackle problems in robotic reinforcement learning can be effective in real-world scenarios.
% successfully optimizes the embeddings and policy parameters, with minimal resets, to perform the new task. 
%%AK: how do higher numbers only say that we can optimize embeddings.
We include a plot of the success rate of the policy during finetuning in the Appendix.
% \begin{itemize}
%     \item Our full method evaluated on the container placing and drawer tasks in the real world, demonstrating that our finetuning method successfully improves the performance of the pretrained policy on a new task.
%     \item Naive forward-backward controller. Offline phase on multi-task data with two extra indices/buffers for the forward and reverse skill. Finetune on new task reset-free assigning data to new indices and also training on prior data. This can be thought of as an ablation of our method with no CEM finetuning. We may want to also show this in sim. 
% \end{itemize}
\fi


\iffalse 

\subsection{How does \methodName\ compare to prior methods that also use minimal resets?}
Next, we compare our system to prior work that has addressed learning with minimal resets and several other instructive variants of our approach. We compare to \textbf{R3L} (\citet{zhu2020ingredients}) which alternates between a forward controller that optimizes a reward for completing the task and a perturbation controller that optimizes a novelty exploration bonus. To perform a fair comparison to our method which has access to prior data, we initialize the forward controller for R3L by performing offline multi-task RL on the same prior data. Then, during online training we label the data passed to the forward controller with an additional task index not used during the offline training. For ablations, we compare to our method applied in the episodic setting (\textbf{ARIEL + resets}) where in the online phase we perform an external reset after every trial. We also compare to an ablation of our method without adaptation of the task embeddings (\textbf{Multi-task RL}). 
%We modify the policy and Q function architectures to accept two additional one-hot task indices. These task indices go unused during offline learning, 
During online training, we label data collected by the forward and backward controller with two additional task indices that were unused in the offline phase. This ablation is similar to standard multi-task RL but with a distinct offline phase where some of the tasks are trained and an online phase where the rest of the tasks are trained.

Figure \ref{fig:reset_free_graphs} shows the results. Only our method succeeds at learning the task, likely due to the difficulty of learning from image observations and sparse rewards. While \textbf{R3L} and the \textbf{Multi-Task RL} ablation both succeeded at learning the tasks in the offline phase (\doubt{see the Appendix for plots of the offline phase} of these baselines), they are unable to make progress on the new task. This is likely because the data collected in the online phase and labeled with a new task index is out of distribution for the policies learned in the offline phase. Thus, these methods cannot use skills learned offline to efficiently explore the new task. Our method solves this challenge with an explicit mechanism for searching in the space of task embeddings, starting from those used during offline learning, to induce better-than-random initial exploratory behavior.


\subsection{Evaluating Sample-Efficiency}
We next evaluate whether our method enables greater sample-efficiency than learning from scratch. We compare our method to simply applying RL to the target task, using the same RL algorithm as our system (\textbf{AWAC (no prior data)}). We also compare to an \textbf{oracle} method which is trained offline on data for a single task and then trained online on the same task. Perhaps unsurprisingly, we found that learning from scratch fails in the challenging setting of learning from images and sparse reward. However, our method learns just as efficiently or more efficiently than the oracle despite learning from offline data for other tasks rather than the same task. Thus, our method demonstrates that properly leveraging prior data can improve sample-efficiency even when data is only available for other tasks.

\subsection{Evaluating Generalization}
Finally, we evaluate whether training on diverse multi-task data encourages learning robust representations that allow the agent to generalize to new conditions without any adaptation. The setting of applying a policy learned under one set of conditions to a new set with no adaptation is known as zero-shot policy transfer. In the real-world container setting we compare the zero-shot performance of our method 

\fi


==> rss/text/7-discussion.tex <==
\section{Discussion}

In this work, we proposed overcoming the numerous challenges of real-world robotic reinforcement learning through better leveraging prior datasets.
While reinforcement learning often involves acquiring a skill from scratch, such a formalism is not well-suited to real world conditions where running online data collection is expensive, and previously collected datasets are often accessible. 
While the use of previously collected datasets for tackling a particular challenge (such as that of sample efficiency~\cite{nair2020accelerating}, or better generalization~\cite{lin2021}) has been addressed in prior work, our work aims to address such challenges jointly in a single robotic learning system, which leverages prior data as the primary mechanism to facilitate autonomy during online training, improve efficiency, and boost generalization. In our experiments, we show that our method is able to make consistent progress in online finetuning despite having to learn from sparse rewards, matching or exceeding the final performance of an oracle baseline that receives prior data \emph{of the actual test task}, and significantly outperforming a baseline without prior data. This supports our central hypothesis that prior data can be a significant facilitator for real-world robotic RL. One limitation of our analysis is that our new online training tasks are structurally quite similar to the prior data used for offline pretraining. While the objects during online training are different, they do not require significantly distinct physical skills. We believe that, as the breadth and diversity of the available prior data increases, the offline pretrained model will correspondingly be useful for a broader range of new tasks. Exploring this direction by scaling up the proposed approach is an exciting avenue for future work.

%\begin{itemize}
 %   \item We could talk about the degenerate behavior we notice where CEM just produces a training task one-hot. This is likely because we have relatively few tasks in the prior data so the latent space is not particularly smooth. With more tasks in the prior data, a continuous optimization procedure like CEM might make more sense.
%\end{itemize}

==> text/3-preliminaries.tex <==
\section{Preliminaries}
\label{sec:prelims}

